FBGEMM: Enabling High-Performance Low-Precision Deep Learning Inference

Deep learning models typically use single-precision (FP32) floating point data types for representing activations and weights, but a slew of recent research work has shown that computations with reduced-precision data types (FP16, 16-bit integers, 8-bit integers or even 4- or 2-bit integers) are enough to achieve same accuracy as FP32 and are much more efficient. Therefore, we designed fbgemm, a high-performance kernel library, from ground up to perform high-performance quantized inference on current generation CPUs. fbgemm achieves efficiency by fusing common quantization operations with a high-performance gemm implementation and by shape- and size-specific kernel code generation at runtime. The library has been deployed at Facebook, where it delivers greater than 2x performance gains with respect to our current production baseline.

==> background.tex <==
\subsection{Why GEMM Efficiency matters}
Fully connected (FC) operators are the biggest consumers of floating point operations (FLOPs) in the deep learning models deployed in Facebook's data centers. We performed data-center-wide profiling for FLOPs usage in representative models running in production here at Facebook. The pie chart below shows the distribution of the deep learning inference FLOPs in our data centers measured over a 24-hour period.


FC operators are just plain GEMM, so overall efficiency directly depends on GEMM efficiency.  Many deep learning frameworks implement convolution as im2col followed by GEMM~\cite{gemmDL}, because performant GEMM implementations are readily available in linear algebra libraries from the high-performance computing (HPC) domain. But straightforward im2col adds overhead from the copy and replication of input data, so some deep learning libraries also implement direct (im2col-free) convolution for improved efficiency. As explained in more detail below, we provide a way to fuse im2col with the main GEMM kernel to minimize im2col overhead. The high-performance GEMM kernel is a critical part, but it's not the only one. In general, there is a mismatch between what HPC libraries provide and the requirements of deep learning inference. HPC libraries usually do not support quantized GEMM-related operations efficiently. They are not optimized for shapes and sizes of matrices common in deep learning inference. And they do not take advantage of the constant nature of the weight matrix.

Deep learning models have typically used FP32 data types for representing activations and weights, but computations with mixed-precision data types (8-bit or 16-bit integers, FP16, etc.) are generally much more efficient. Recent industry and research works have shown that inference using mixed-precision works well without adversely affecting accuracy. \fbgemm{} uses this alternative strategy and improves inference performance with quantized models. Furthermore, newer generations of GPUs, CPUs, and specialized tensor processors natively support lower-precision compute primitives, such as FP16/INT8 in Nvidia tensor cores or INT8 in Google processors. So the deep learning community is moving toward low-precision models. This movement indicates that quantized inference is a step in the right direction, and \fbgemm{} provides a way to perform efficient quantized inference on current and upcoming generation of CPUs.


